Reasoning about the Impacts of Information Sharing

In this paper we describe a decision process framework allowing an agent to decide what information it should reveal to its neighbours within a communication graph in order to maximise its utility. We assume that these neighbours can pass information onto others within the graph. The inferences made by agents receiving the messages can have a positive or negative impact on the information providing agent, and our decision process seeks to identify how a message should be modified in order to be most beneficial to the information producer. Our decision process is based on the provider's subjective beliefs about others in the system, and therefore makes extensive use of the notion of trust. Our core contributions are therefore the construction of a model of information propagation; the description of the agent's decision procedure; and an analysis of some of its properties.

==> journal-version_arxiv-19Nov2013/symbols-yuqing.tex <==
\newcommand{\vsim}{\mathrel{{|}\mspace{-3mu}{\sim}}}
\newcommand{\tx}[1]{\textrm{#1}}

\newcommand{\myFALSE}{\tx{FALSE}}
\newcommand{\myTRUE}{\tx{TRUE}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcSS}{\mathcal{S}'}
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcsR}{\mcR} %specification/input relation
\newcommand{\mclR}{\underline{\mcR}}
\newcommand{\mclM}{\underline{\mcM}}
\newcommand{\lpi}{\underline{\pi}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\myV}{\msf{VAR}}
\newcommand{\mcOP}{\mathcal{O}\mathcal{P}}
\newcommand{\mcDF}{\mathcal{D}\mathcal{F}}
\newcommand{\mcCE}{\mathcal{C}\mathcal{E}}
\newcommand{\mcBE}{\mathcal{B}\mathcal{E}}
\newcommand{\mcIR}{\mathcal{I}\mathcal{R}}
\newcommand{\mcSPL}{\mathcal{S}\mathcal{P}\mathcal{L}}
%\newcommand{\mcSASPL}{SA\mathcal{S}\mathcal{P}\mathcal{L}}
\newcommand{\mcSADEF}{SA\mathcal{D}\mathcal{E}\mathcal{F}}
\newcommand{\mcSPEC}{\mathcal{S}\mathcal{P}\mathcal{E}\mathcal{C}}
\newcommand{\myType}{\msf{type}}
\newcommand{\myPred}{\msf{Pred}}
\newcommand{\myP}{\mcP}
\newcommand{\myLayer}{\msf{layer}}
\newcommand{\myLevel}{\msf{level}}
\newcommand{\myLevelVector}{\msf{levelVector}}
\newcommand{\nextS}{S'}
\newcommand{\mcSA}{\mcS\mcA}
\newcommand{\mcFRM}{\mc{F}\mc{R}\mc{M}}
%truth conditionals
\newcommand{\mcTC}{\mc{T}\mc{C}}

\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcZ}{\mathcal{Z}}


%---
%For argumentation
\newcommand{\myL}{\mathcal{L}}
%\newcommand{\myArg}{\mathcal{A}\mathcal{R}\mathcal{G}}
\newcommand{\myArg}{\msf{A}\msf{R}\msf{G}}
%\newcommand{\myArgFW}{\myArg\mc{F}\mc{W}}
\newcommand{\myArgFW}{\msf{A}\msf{F}}
%argumentation framework
\newcommand{\myAF}{\msf{A}\msf{F}}
%argumentation system
%\newcommand{\myAS}{\msf{A}\msf{S}}
\newcommand{\myAFP}{\myAF\msf{P}}
\newcommand{\myAFD}{\myAF\msf{D}}
\newcommand{\myAT}{\myArg}
\newcommand{\myA}{\myAT}
%inference patterns/labels
\newcommand{\myRS}{\mc{R}\mc{S}}
%\newcommand{\myD}{\mathcal{D}\mathcal{F}\mathcal{T}}
\newcommand{\myD}{\msf{D}\msf{F}\msf{T}}
\newcommand{\myDFD}{\msf{D}\msf{F}\msf{D}}
\newcommand{\myPD}{\msf{P}\msf{D}\msf{F}\msf{T}}
\newcommand{\myK}{\mbf{K}}
%\newcommand{\myKMRC}{\msf{KMRC}}
\newcommand{\myKL}{\msf{KL}}
\newcommand{\myKR}{\msf{KR}}
\newcommand{\myKI}{\msf{KI}}
\newcommand{\myKG}{\msf{KG}}
\newcommand{\myRebut}{\msf{rebut}}
\newcommand{\myUndercut}{\msf{undercut}}
\newcommand{\myContradict}{\msf{contradict}}
\newcommand{\myC}{\mbf{C}}
\newcommand{\myKP}{\msf{KPREF}}
\newcommand{\myKM}{\msf{KM}}
\newcommand{\myFarg}{\msf{F}_{arg}}
\newcommand{\myS}{{\underline{\msf{S}}}}
%\newcommand{\myPref}{\mc{P}\mc{R}\mc{E}\mc{F}}
\newcommand{\myPref}{\msf{P}\msf{R}\msf{E}\msf{F}}
\newcommand{\myAS}{\msf{A}\msf{S}}
\newcommand{\myASID}{\msf{A}\msf{S}\msf{ID}}
\newcommand{\myASPremise}{\msf{A}\msf{S}\msf{Premise}}
\newcommand{\myASSupport}{\msf{A}\msf{S}\msf{Support}}
\newcommand{\myASConclusion}{\msf{A}\msf{S}\msf{Conclusion}}
\newcommand{\myASUndercuts}{\msf{A}\msf{S}\msf{Undercuts}}
\newcommand{\myASRebuts}{\msf{A}\msf{S}\msf{Rebuts}}
\newcommand{\myASPref}{\msf{A}\msf{S}\msf{Pref}}
\newcommand{\myVarList}{\msf{VarList}}
\newcommand{\myName}{\msf{name}}
\newcommand{\myASCombine}{\msf{ASCombine}}

%----


%---
%For dialogues
\newcommand{\mcDP}{\mcD\mathcal{P}}
\newcommand{\mcDS}{\mcD\mathcal{S}}
\newcommand{\mcDSS}{\mcD\mathcal{S}'}
\newcommand{\mcDA}{\mcD\mathcal{A}}
\newcommand{\mcDM}{\mcD\mathcal{M}}
\newcommand{\mcDR}{\mcD\mathcal{R}}
\newcommand{\mcDOP}{\mcD\mathcal{O}\mathcal{P}}
\newcommand{\mcDDF}{\mcD\mathcal{D}\mathcal{F}}
\newcommand{\mcDCE}{\mcD\mathcal{C}\mathcal{E}}
\newcommand{\mcDIR}{\mcD\mathcal{I}\mathcal{R}}
\newcommand{\mclDR}{\overline{\mcDR}}
%---


%For cognitive systems
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcCP}{\mcC\mathcal{P}}
\newcommand{\mcCS}{\mcC\mathcal{S}}
\newcommand{\mcCSS}{\mcC\mathcal{S}'}
\newcommand{\percept}{PERCEPT}
%\newcommand{\mcCA}{\mcD\mathcal{A}}
%\newcommand{\mcCM}{\mcD\mathcal{M}}
%\newcommand{\mcCR}{\mcD\mathcal{R}}
\newcommand{\cogs}{cogs}
%---


\newcommand{\h}[1]{\hat{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\mch}[1]{\wh{\mathcal{#1}}}
\newcommand{\mchP}{\mch{P}}
\newcommand{\mchS}{\mch{S}}
\newcommand{\mchSS}{\mch{S}'}
\newcommand{\mchA}{\mch{A}}
\newcommand{\mchM}{\mch{M}}
\newcommand{\mchR}{\mch{R}}


\newcommand{\vx}{\vec{x}}
\newcommand{\vP}{\vec{P}}
\newcommand{\vQ}{\vec{Q}}
\newcommand{\vy}{\vec{y}}

%agent
%\newcommand{\ag}{\msf{Ag}}
%agent system
\newcommand{\ags}{\msf{AGS}}


%trust
\newcommand{\trust}{\msf{trust}}
\newcommand{\bel}{\msf{Bel}}
\newcommand{\s}{\msf{s}}

%ontology
\newcommand{\mcO}{\mc{O}}
\newcommand{\Tbox}{\msf{Tbox}}
\newcommand{\Abox}{\msf{Abox}}
\newcommand{\myKB}{\msf{KB}}
\newcommand{\myAns}{\msf{ANS}}

%---
%norm
%MoDals/norm meta symbols
\newcommand{\md}{\msf{M}\msf{D}}
\newcommand{\nd}{\msf{M}\msf{D}}
%Norm names
\newcommand{\nm}{\msf{N}\msf{M}}
%---

\newcommand{\biarrow}{\leftrightarrow}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}%\hbox{\equalsfill}}}

%---
%from Simon's file
\newcommand{\PSL}[3]{\ANNOT{#1}\begin{array}[b]{c}#2\\ \hline #3\end{array}}
\newcommand{\ANNOT}[1]{\mbox{$\ {}^{^{\mbox{\rm \footnotesize#1}}}$}}
\newcommand{\Sequent}[2]{\mbox{$#1\tcr#2$}}
\newcommand{\tcr}{\vdash_{TCR}}
\newcommand{\SP}{\makebox[.1cm]{\ }}
\newcommand{\mrm}[1]{\mbox{$ {}^{^{\mbox{\rm \footnotesize#1}}}$}}
%----




